Functional A Posteriori Error Equalities for Conforming Mixed Approximations of Elliptic Problems

In this paper we show how to find the exact error (not just an estimate of the error) of a conforming mixed approximation by using the functional type a posteriori error estimates in the spirit of Repin. The error is measured in a mixed norm which takes into account both the primal and dual variables. We derive this result for elliptic partial differential equations of a certain class. We first derive a special version of our main result by using a simplified reaction-diffusion problem to demonstrate the strong connection to the classical functional a posteriori error estimates of Repin. After this we derive the main result in an abstract setting. Our main result states that in order to obtain the exact global error value of a conforming mixed approximation one only needs the problem data and the mixed approximation of the exact solution. There is no need for calculating any auxiliary data. The calculation of the exact error consists of simply calculating two (usually integral) quantities where all the quantities are known after the approximate solution has been obtained by any conforming method. We also show some numerical computations to confirm the results.

==> head_paper.tex <==

\usepackage{a4,exscale,ifthen,amsfonts,amssymb,amsmath,amscd,graphicx}
\usepackage[english]{babel}
\usepackage[mathscr]{eucal}

\setlength{\textwidth}{16cm}
\setlength{\textheight}{22cm}
\setlength{\oddsidemargin}{-0.1cm}
\setlength{\evensidemargin}{-0.1cm}

\author{{\sf\pauthor}}
\pagestyle{myheadings}
\markboth{\pauthor}{\shorttitle}

\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\setcounter{footnote}{1}
\numberwithin{equation}{section}

\newenvironment{acknow}{{\vspace*{1cm}\noindent\bf Acknowledgements }}{}
\newcommand{\bewboxw}{\mbox{}\hfill $\square$ \\}
\newcommand{\bewboxb}{\mbox{}\hfill $\blacksquare$ \\}
\newenvironment{proof}{{\noindent\bf Proof }}{\bewboxw}
\newenvironment{proofof}[1]{{\noindent\bf Proof of #1 }}{\bewboxw}

\newcommand{\keywords}[1]{{\noindent\bf Key Words }#1}
\newcommand{\amsclass}[1]{{\noindent\bf AMS MSC-Classifications }#1}

\ifthenelse{\equal{\mylabelonoff}{on}}
{\newcommand{\mylabel}[1]{\label{#1}\fbox{{\rm #1}}}}{\newcommand{\mylabel}[1]{\label{#1}\makebox[0mm][]{}}}
\ifthenelse{\equal{\allowdisbrk}{yes}}
{\allowdisplaybreaks}{}

\newcommand{\paper}[7]{\bibitem{#1} #2, `#3', {\it #4}, #5, (#6), #7.}
\newcommand{\paperpub}[5]{\bibitem{#1} #2, `#3', {\it #4}, (#5), accepted for publication.}
\newcommand{\paperpre}[4]{\bibitem{#1} #2, `#3', (#4), in preparation.}
\newcommand{\papersub}[4]{\bibitem{#1} #2, `#3', (#4), submitted.}
\newcommand{\book}[6]{\bibitem{#1} #2, {\it #3}, #4, #5, (#6).}
\newcommand{\diss}[5]{\bibitem{#1} #2, `#3', {\sf Dissertation}, #4, (#5).}
\newcommand{\dissavail}[6]{\bibitem{#1} #2, `#3', {\sf Dissertation}, #4, (#5), available from {\tt #6}.}
\newcommand{\habil}[5]{\bibitem{#1} #2, `#3', {\sf Habilitationsschrift}, #4, (#5).}
\newcommand{\habilavail}[6]{\bibitem{#1} #2, `#3', {\sf Habilitationsschrift}, #4, (#5), available from {\tt #6}.}
\newcommand{\dipl}[5]{\bibitem{#1} #2, `#3', {\sf Diplomarbeit}, #4, (#5).}
\newcommand{\diplavail}[6]{\bibitem{#1} #2, `#3', {\sf Diplomarbeit}, #4, (#5), available from {\tt #6}.}
\newcommand{\repjyu}[8]{\bibitem{#1} #2, `#3', {\it Reports of the Department of Mathematical Information Technology}, 
University of Jyv\"askyl\"a, Series #4. Scientific Computing, No. #4. #5/#6, ISBN #7, ISSN #8.}
\newcommand{\reportavail}[7]{\bibitem{#1} #2, `#3', {\it #4}, #5, (#6), available from {\tt #7}.}
\newcommand{\preprintarxiv}[5]{\bibitem{#1} #2, `#3', (#4), preprint, available at {\tt arXiv}: #5.}


==> head_paule.tex <==

%%%%%%%%%%%%%%%%%%%%%
% LaTeX header file %
% Dirk Pauly        %
%%%%%%%%%%%%%%%%%%%%%

\usepackage[mathscr]{eucal}
\usepackage{color}
% \usepackage{graphicx}

\def\rc{\color{red}}
\def\gc{\color{green}}

\newcommand{\Abb}[5]{\begin{array}{ccccc}#1&:&#2&\longrightarrow&#3\\{}&{}&#4&\longmapsto&#5\end{array}}
\newcommand{\ds}{\displaystyle}
\newcommand{\ol}{\overline}
\newcommand{\ul}{\underline}
\newcommand{\ub}{\underbrace}
\newcommand{\ob}{\overbrace}
\newcommand{\nz}{\mathbb{N}}
\newcommand{\zz}{\mathbb{Z}}
\newcommand{\nzz}{\nz_{0}}
\newcommand{\rz}{\mathbb{R}}
\newcommand{\rzp}{\rz_{+}}
\newcommand{\rzm}{\rz_{-}}
\newcommand{\rzpm}{\rz_{\pm}}
\newcommand{\rt}{\rz^3}
\newcommand{\rttt}{\rz^{3\times3}}
\newcommand{\rttts}{\rttt_{\sym}}
\newcommand{\rN}{\rz^N}
\newcommand{\rNtN}{\rz^{N\times N}}
\newcommand{\rNtNs}{\rNtN_{\sym}}
\newcommand{\dd}{\text{d}}
\newcommand{\intl}{\,\dd\lambda}
\DeclareMathOperator{\p}{\partial}
\newcommand{\pt}{\p_{t}}
\newcommand{\na}{\nabla}
\newcommand{\nas}{\na'}
\newcommand{\nac}{\overset{\circ}{\na}}
%\newcommand{\nag}{\na_{\Gamma}}
\newcommand{\nag}{\widetilde{\na}}
\newcommand{\nat}{\trans{\na}}
\DeclareMathOperator{\ed}{d}
\DeclareMathOperator{\eD}{D}
\DeclareMathOperator{\cd}{\delta}
\DeclareMathOperator{\cD}{\Delta}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Grad}{Grad}
\DeclareMathOperator{\cograd}{cograd}
\DeclareMathOperator{\CoGrad}{CoGrad}
\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\Rot}{Rot}
\DeclareMathOperator{\rotc}{\overset{\circ}{\rot}}
\DeclareMathOperator{\curl}{curl}
\DeclareMathOperator{\Curl}{Curl}
\DeclareMathOperator{\curlga}{curl_{\ga}}
\DeclareMathOperator{\Curlga}{Curl_{\ga}}
\renewcommand{\div}{\operatorname{div}}
\newcommand{\divc}{\overset{\circ}{\div}}
\DeclareMathOperator{\Div}{Div}
%\newcommand{\divg}{\div_{\Gamma}}
%\newcommand{\rotg}{\rot_{\Gamma}}
\newcommand{\divg}{\widetilde{\div}}
\newcommand{\rotg}{\widetilde{\rot}}
\DeclareMathOperator{\iu}{i}
\DeclareMathOperator{\euler}{e}
\newcommand{\trans}[1]{{#1}^\top}
% \newcommand{\trans}[1]{{#1}^t}
% \newcommand{\trans}[1]{{#1}^T}
% \DeclareMathOperator{\T}{T}
\newcommand{\T}{T}
\newcommand{\TS}{S}
\newcommand{\TR}{R}
\newcommand{\Tp}{P}
\newcommand{\TP}{P}
\newcommand{\TF}{F}
\newcommand{\Tskew}{S}
\newcommand{\eps}{\varepsilon}
\newcommand{\epsmo}{\eps^{-1}}
\newcommand{\mumo}{\mu^{-1}}
\newcommand{\muu}{\ul{\mu}}
\newcommand{\muo}{\ol{\mu}}
\newcommand{\epsu}{\ul{\eps}}
\newcommand{\epso}{\ol{\eps}}
\newcommand{\epsh}{\hat{\eps}}
\newcommand{\epst}{\trans{\eps}}
\newcommand{\sigmap}{\sigma_{\mathtt{p}}}
\newcommand{\om}{\Omega}
\newcommand{\oms}{\omega}
\newcommand{\pom}{\p\!\om}
\newcommand{\poms}{\p\!\oms}
\newcommand{\omb}{\ol{\om}}
\newcommand{\ga}{\Gamma}
\newcommand{\gas}{\gamma}
\newcommand{\gat}{\ga_{t}}
\newcommand{\gan}{\ga_{n}}
\newcommand{\gatj}{\ga_{t,j}}
\newcommand{\ttrga}{\tau_{\ga}}
\newcommand{\ttrgat}{\tau_{\gat}}
\newcommand{\ttrgatj}{\tau_{\gatj}}
\newcommand{\ntrgan}{\nu_{\gan}}
\def\intO{\int_{\om}}
\newcommand{\equi}{\Leftrightarrow}
\def\impl{\Rightarrow}
\def\lpmi{\Leftarrow}
\newcommand{\qequi}{\quad\equi\quad}
\newcommand{\qqequi}{\qquad\equi\qquad}
\newcommand{\qimpl}{\quad\impl\quad}
\newcommand{\qqimpl}{\qquad\impl\qquad}
\def\e{\mathrm{e}}
\DeclareMathOperator{\Lin}{Lin}
\DeclareMathOperator{\loc}{loc}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\sym}{sym}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\tr}{tr}
\renewcommand{\skew}{\operatorname{skew}}
\newcommand{\zvec}[2]{\begin{bmatrix}#1\\#2\end{bmatrix}}
\newcommand{\dvec}[3]{\begin{bmatrix}#1\\#2\\#3\end{bmatrix}}
\newcommand{\zmat}[4]{\begin{bmatrix}#1&#2\\#3&#4\end{bmatrix}}
\newcommand{\dmat}[9]{\begin{bmatrix}#1&#2&#3\\#4&#5&#6\\#7&#8&#9\end{bmatrix}}
\DeclareMathOperator{\id}{id}
\newcommand{\dl}{\,d\lambda}
\newcommand{\dlo}{\,do}
\DeclareMathOperator{\SO}{SO}
\DeclareMathOperator{\so}{\mathfrak{so}}
\DeclareMathOperator{\dev}{dev}
\def\set#1#2{\{#1\,:\,#2\}}
\def\Set#1#2{\left\{#1\,:\,#2\right\}}

\newcommand{\ch}{\hat{c}}
\newcommand{\ct}{\tilde{c}}
\newcommand{\cb}{\bar{c}}
\newcommand{\cc}{\check{c}}
\newcommand{\cp}{c_{\mathtt{p}}}
\newcommand{\cpc}{c_{\mathtt{p},\circ}}
\newcommand{\cpq}{c_{\mathtt{p},q}}
\newcommand{\cpqmo}{c_{\mathtt{p},q-1}}
\newcommand{\cpqpo}{c_{\mathtt{p},q+1}}
\newcommand{\cpz}{c_{\mathtt{p},0}}
\newcommand{\cpeps}{c_{\mathtt{p},\eps}}
\newcommand{\cpzeps}{c_{\mathtt{p},0,\eps}}
\newcommand{\cpo}{c_{\mathtt{p},1}}
\newcommand{\cm}{c_{\mathtt{m}}}
\newcommand{\cme}{c_{\mathtt{m,e}}}
\newcommand{\cmt}{c_{\mathtt{m,t}}}
\newcommand{\cmteps}{c_{\mathtt{m,t},\eps}}
\newcommand{\cmtid}{c_{\mathtt{m,t},\id}}
\newcommand{\cmrot}{c_{\mathtt{m},\rot}}
\newcommand{\cmtrot}{c_{\mathtt{m,t},\rot}}
\newcommand{\cmtdiv}{c_{\mathtt{m,t},\div}}
\newcommand{\cmtroteps}{c_{\mathtt{m,t},\rot,\eps}}
\newcommand{\cmtrotepsmu}{c_{\mathtt{m,t},\rot,\eps,\mu}}
\newcommand{\cmtrotepsid}{c_{\mathtt{m,t},\rot,\eps,\id}}
\newcommand{\cmtrotidid}{c_{\mathtt{m,t},\rot,\id,\id}}
\newcommand{\cmtdiveps}{c_{\mathtt{m,t},\div,\eps}}
\newcommand{\ctme}{\tilde{c}_{\mathtt{m,e}}}
\newcommand{\ctmt}{\tilde{c}_{\mathtt{m,t}}}
\newcommand{\cmm}{c_{\mathtt{m,m}}}
\newcommand{\cmn}{c_{\mathtt{m,n}}}
\newcommand{\cmneps}{c_{\mathtt{m,n},\eps}}
\newcommand{\cmnid}{c_{\mathtt{m,n},\id}}
\newcommand{\cmnmu}{c_{\mathtt{m,n},\mu}}
\newcommand{\cmnrot}{c_{\mathtt{m,n},\rot}}
\newcommand{\cmndiv}{c_{\mathtt{m,n},\div}}
\newcommand{\cmnroteps}{c_{\mathtt{m,n},\rot,\eps}}
\newcommand{\cmnrotepsmu}{c_{\mathtt{m,n},\rot,\eps,\mu}}
\newcommand{\cmnrotepsid}{c_{\mathtt{m,n},\rot,\eps,\id}}
\newcommand{\cmnrotideps}{c_{\mathtt{m,n},\rot,\id,\eps}}
\newcommand{\cmnrotidid}{c_{\mathtt{m,n},\rot,\id,\id}}
\newcommand{\cmndiveps}{c_{\mathtt{m,n},\div,\eps}}
\newcommand{\ctmm}{\tilde{c}_{\mathtt{m,m}}}
\newcommand{\ctmn}{\tilde{c}_{\mathtt{m,n}}}
\newcommand{\cf}{c_{\mathtt{f}}}
\newcommand{\cpf}[1]{c_{\mathtt{pf},#1}}
\newcommand{\ck}{c_{\mathtt{k}}}
\newcommand{\ckF}{c_{\mathtt{k},\TF}}
\newcommand{\ckt}{c_{\mathtt{k},t}}
\newcommand{\cktF}{c_{\mathtt{k},t,\TF}}
\newcommand{\cks}{c_{\mathtt{k},s}}
\newcommand{\cksF}{c_{\mathtt{k},s,\TF}}
\newcommand{\cktj}{c_{\mathtt{k},t,j}}
\newcommand{\cksj}{c_{\mathtt{k},s,j}}
\newcommand{\ckemp}{c_{\mathtt{k},\emptyset}}
\newcommand{\ckjemp}{c_{\mathtt{k},j,\emptyset}}
\newcommand{\chemp}{\ch_{\emptyset}}
\newcommand{\chF}{\ch_{\TF}}
\newcommand{\cF}{c_{\TF}}
\newcommand{\cN}{c_{N}}
\newcommand{\cNa}{c_{N,\alpha}}

\newcommand{\ot}{\leftarrow}
\newcommand{\wto}{\rightharpoonup}
\newcommand{\wot}{\leftharpoonup}
\newcommand{\compemb}{\hookrightarrow}

\def\ut{\tilde{u}}
\def\uh{\hat{u}}
\def\ub{\bar{u}}
\def\uc{\check{u}}
\def\vt{\tilde{v}}
\def\vh{\hat{v}}
\def\vb{\bar{v}}
\def\vc{\check{v}}
\def\Ht{\tilde{H}}
\def\Hh{\hat{H}}
\def\Hb{\bar{H}}
\def\Hc{\check{H}}
\def\Et{\tilde{E}}
\def\Eh{\hat{E}}
\def\Eb{\bar{E}}
\def\Ec{\check{E}}
\def\et{\tilde{e}}
\def\eh{\hat{e}}
\def\eb{\bar{e}}
\def\ec{\check{e}}

\def\calM{\mathcal{M}}
\def\calE{\mathcal{E}}
\def\calA{\mathcal{A}}
\def\calB{\mathcal{B}}
\def\cE{\mathcal{E}}
\def\cR{\mathcal{R}}

\DeclareMathOperator{\Lebesgue}{\mathsf{L}}
\newcommand{\Lgen}[2]{\Lebesgue^{#1}_{#2}}
\def\Li{\Lgen{\infty}{}}
\def\Liom{\Li(\om)}
\def\Lo{\Lgen{1}{}}
\def\Loom{\Lo(\om)}
\def\Lt{\Lgen{2}{}}
\def\Lteps{\Lgen{2}{\eps}}
\def\Ltmu{\Lgen{2}{\mu}}
\def\Ltom{\Lt(\om)}
\def\Ltoms{\Lt(\oms)}
\def\Ltepsom{\Lgen{2}{\eps}(\om)}
\def\Ltepsoms{\Lgen{2}{\eps}(\oms)}
\def\Ltmuom{\Lgen{2}{\mu}(\om)}
\def\Ltmuoms{\Lgen{2}{\mu}(\oms)}
\def\Ltsym{\Lgen{2}{\sym}}
\def\Ltsymom{\Ltsym(\om)}
\def\Ltga{\Lt(\ga)}
\def\Ltgat{\Lt(\gat)}
\def\Lq{\Lgen{q}{}}
\def\Lqom{\Lq(\om)}
\def\Lp{\Lgen{p}{}}
\def\Lpom{\Lp(\om)}

\def\Ltloc{\Lgen{2}{\loc}}
\def\Lts{\Lgen{2}{s}}
\def\Ltspo{\Lgen{2}{s+1}}
\def\Ltsmo{\Lgen{2}{s-1}}
\def\Ltmo{\Lgen{2}{-1}}
\def\Ltz{\Lgen{2}{0}}
\def\Ltpo{\Lgen{2}{1}}
\def\Ltlocom{\Ltloc(\om)}
\def\Ltsom{\Lts(\om)}
\def\Ltspoom{\Ltspo(\om)}
\def\Ltsmoom{\Ltsmo(\om)}
\def\Ltmoom{\Ltmo(\om)}
\def\Ltzom{\Ltz(\om)}
\def\Ltpoom{\Ltpo(\om)}

\newcommand{\qLt}[1]{\Lgen{2,#1}{}}
\newcommand{\Ltq}{\qLt{q}}
\newcommand{\Ltqpo}{\qLt{q+1}}
\newcommand{\Ltqmo}{\qLt{q-1}}
\newcommand{\Ltqom}{\Ltq(\om)}
\newcommand{\Ltqpoom}{\Ltqpo(\om)}
\newcommand{\Ltqmoom}{\Ltqmo(\om)}

\DeclareMathOperator{\DSobolev}{\mathsf{D}}
\newcommand{\Dgen}[3]{\overset{#3}{\DSobolev}{}^{#1}_{#2}}
\newcommand{\qD}[1]{\Dgen{#1}{}{}}
\newcommand{\qDz}[1]{\Dgen{#1}{0}{}}
\newcommand{\qDc}[1]{\Dgen{#1}{}{\circ}}
\newcommand{\qDcz}[1]{\Dgen{#1}{0}{\circ}}
\newcommand{\Dq}{\qD{q}}
\newcommand{\Dqpo}{\qD{q+1}}
\newcommand{\Dqmo}{\qD{q-1}}
\newcommand{\Dqz}{\qDz{q}}
\newcommand{\Dqpoz}{\qDz{q+1}}
\newcommand{\Dqmoz}{\qDz{q-1}}
\newcommand{\Dqc}{\qDc{q}}
\newcommand{\Dqpoc}{\qDc{q+1}}
\newcommand{\Dqmoc}{\qDc{q-1}}
\newcommand{\Dqcz}{\qDcz{q}}
\newcommand{\Dqpocz}{\qDcz{q+1}}
\newcommand{\Dqmocz}{\qDcz{q-1}}
\newcommand{\Dqom}{\Dq(\om)}
\newcommand{\Dqpoom}{\Dqpo(\om)}
\newcommand{\Dqmoom}{\Dqmo(\om)}
\newcommand{\Dqzom}{\Dqz(\om)}
\newcommand{\Dqpozom}{\Dqpoz(\om)}
\newcommand{\Dqmozom}{\Dqmoz(\om)}
\newcommand{\Dqcom}{\Dqc(\om)}
\newcommand{\Dqpocom}{\Dqpoc(\om)}
\newcommand{\Dqmocom}{\Dqmoc(\om)}
\newcommand{\Dqczom}{\Dqcz(\om)}
\newcommand{\Dqpoczom}{\Dqpocz(\om)}
\newcommand{\Dqmoczom}{\Dqmocz(\om)}
\newcommand{\Dqcgatom}{\Dqc(\gat,\om)}
\newcommand{\Dqczgatom}{\Dqcz(\gat,\om)}
\newcommand{\Dqmocgatom}{\Dqmoc(\gat,\om)}
\newcommand{\Dqmoczgatom}{\Dqmocz(\gat,\om)}
\newcommand{\Dqpoczgatom}{\Dqpocz(\gat,\om)}
\newcommand{\Dqczganom}{\Dqcz(\gan,\om)}
\newcommand{\Dqmocganom}{\Dqmoc(\gan,\om)}

\DeclareMathOperator{\DeSobolev}{\Delta}
\newcommand{\Degen}[3]{\overset{#3}{\DeSobolev}{}^{#1}_{#2}}
\newcommand{\qDe}[1]{\Degen{#1}{}{}}
\newcommand{\qDec}[1]{\Degen{#1}{}{\circ}}
\newcommand{\qDez}[1]{\Degen{#1}{0}{}}
\newcommand{\qDecz}[1]{\Degen{#1}{0}{\circ}}
\newcommand{\Deq}{\qDe{q}}
\newcommand{\Deqpo}{\qDe{q+1}}
\newcommand{\Deqmo}{\qDe{q-1}}
\newcommand{\Deqc}{\qDec{q}}
\newcommand{\Deqpoc}{\qDec{q+1}}
\newcommand{\Deqmoc}{\qDec{q-1}}
\newcommand{\Deqz}{\qDez{q}}
\newcommand{\Deqpoz}{\qDez{q+1}}
\newcommand{\Deqmoz}{\qDez{q-1}}
\newcommand{\Deqcz}{\qDecz{q}}
\newcommand{\Deqpocz}{\qDecz{q+1}}
\newcommand{\Deqmocz}{\qDecz{q-1}}
\newcommand{\Deqom}{\Deq(\om)}
\newcommand{\Deqpoom}{\Deqpo(\om)}
\newcommand{\Deqmoom}{\Deqmo(\om)}
\newcommand{\Deqcom}{\Deqc(\om)}
\newcommand{\Deqpocom}{\Deqpoc(\om)}
\newcommand{\Deqmocom}{\Deqmoc(\om)}
\newcommand{\Deqzom}{\Deqz(\om)}
\newcommand{\Deqpozom}{\Deqpoz(\om)}
\newcommand{\Deqmozom}{\Deqmoz(\om)}
\newcommand{\Deqczom}{\Deqcz(\om)}
\newcommand{\Deqpoczom}{\Deqpocz(\om)}
\newcommand{\Deqmoczom}{\Deqmocz(\om)}
\newcommand{\Deqcganom}{\Deqc(\gan,\om)}
\newcommand{\Deqpocganom}{\Deqpoc(\gan,\om)}
\newcommand{\Deqczganom}{\Deqcz(\gan,\om)}
\newcommand{\Deqmoczganom}{\Deqmocz(\gan,\om)}
\newcommand{\Deqczgatom}{\Deqcz(\gat,\om)}
\newcommand{\Deqpocgatom}{\Deqpoc(\gat,\om)}

\DeclareMathOperator{\Sobolev}{\mathsf{H}}
\newcommand{\Hgen}[3]{\overset{#3}{\Sobolev}{}^{#1}_{#2}}
\def\Ho{\Hgen{1}{}{}}
\def\Ht{\Hgen{2}{}{}}
\def\Hm{\Hgen{m}{}{}}
\def\Hk{\Hgen{k}{}{}}
\def\Hoom{\Ho(\om)}
\def\Htom{\Ht(\om)}
\def\Hmom{\Hm(\om)}
\def\Hkom{\Hk(\om)}
\def\Hoot{\Hgen{1/2}{}{}}
\def\Hootom{\Hoot(\om)}
\def\Hmoot{\Hgen{-1/2}{}{}}
\def\HootG{\Hoot(\Gamma)}
\def\HmootG{\Hmoot(\Gamma)}
\def\Hoc{\Hgen{1}{}{\circ}}
\def\Hkc{\Hgen{k}{}{\circ}}
\def\Hocom{\Hoc(\om)}
\def\Hkcom{\Hkc(\om)}
\def\Hocgatom{\Hoc(\gat;\om)}
\def\Hocganom{\Hoc(\gan;\om)}
\def\Hoz{\Hoc}
\def\Hozom{\Hocom}
\def\Hozgatom{\Hocgatom}
\def\Hoq{\Hgen{1,q}{}{}}
\def\Hoqc{\Hgen{1,q}{}{\circ}}
\def\Hoqom{\Hoq(\om)}
\def\Hoqcom{\Hoqc(\om)}
\def\Hkq{\Hgen{k,q}{}{}}
\def\Hkqc{\Hgen{k,q}{}{\circ}}
\def\Hkqom{\Hkq(\om)}
\def\Hkqcom{\Hkqc(\om)}

\def\Homo{\Hgen{1}{-1}{}}
\def\Hocmo{\Hgen{1}{-1}{\circ}}
\def\Homoom{\Homo(\om)}
\def\Hocmoom{\Hocmo(\om)}

\DeclareMathOperator{\WSobolev}{\mathsf{W}}
\newcommand{\Wgen}[3]{\overset{#3}{\WSobolev}{}^{#1}_{#2}}
\newcommand{\Wo}[1]{\Wgen{1,#1}{}{}}
\newcommand{\Woc}[1]{\Wgen{1,#1}{}{\circ}}
\newcommand{\Woom}[1]{\Wo{#1}(\om)}
\newcommand{\Wocom}[1]{\Woc{#1}(\om)}

\DeclareMathOperator{\Cont}{\mathsf{C}}
\newcommand{\Cgen}[2]{\overset{#2}{\Cont}{}^{#1}}
\def\Cz{\Cgen{0}{}}
\def\Czom{\Cz(\om)}
\def\Czomb{\Cz(\ol{\om})}
\def\Ci{\Cgen{\infty}{}}
\def\Cic{\Cgen{\infty}{\circ}}
\def\Ciq{\Cgen{\infty,q}{}}
\def\Ciqc{\Cgen{\infty,q}{\circ}}
\def\Ciqpo{\Cgen{\infty,q+1}{}}
\def\Ciqpoc{\Cgen{\infty,q+1}{\circ}}
\def\Ciqmo{\Cgen{\infty,q-1}{}}
\def\Ciqmoc{\Cgen{\infty,q-1}{\circ}}
\def\Co{\Cgen{1}{}}
\def\Coc{\Cgen{1}{\circ}}
\def\Ciom{\Ci(\om)}
\def\Cicom{\Cic(\om)}
\def\Ciqom{\Ciq(\om)}
\def\Ciqcom{\Ciqc(\om)}
\def\Ciqpoom{\Ciqpo(\om)}
\def\Ciqpocom{\Ciqpoc(\om)}
\def\Ciqmoom{\Ciqmo(\om)}
\def\Ciqmocom{\Ciqmoc(\om)}
\def\Cicgatom{\Cic(\gat,\om)}
\def\Cicganom{\Cic(\gan,\om)}
\def\Ciqcgatom{\Ciqc(\gat,\om)}
\def\Ciqcganom{\Ciqc(\gan,\om)}
\def\Coom{\Co(\om)}
\def\Cocom{\Coc(\om)}

\DeclareMathOperator{\dirichlet}{\mathcal{H}}
\newcommand{\qharmdi}[2]{\dirichlet^{#1}_{#2}(\om)}
\newcommand{\harmdi}{\qharmdi{}{}}
\newcommand{\harmdiz}{\qharmdi{0}{}}
\newcommand{\harmdio}{\qharmdi{1}{}}
\newcommand{\harmdiq}{\qharmdi{q}{}}
\newcommand{\harmdiqpo}{\qharmdi{q+1}{}}
\newcommand{\harmdiqmo}{\qharmdi{q-1}{}}
\newcommand{\harmdieps}{\qharmdi{}{\eps}}
\newcommand{\harmdiqeps}{\qharmdi{q}{\eps}}

% \newcommand{\Hggen}[3]{\overset{#2}{\Sobolev}{}_{#1}(\grad;#3)}
% \newcommand{\HGgen}[3]{\overset{#2}{\Sobolev}{}_{#1}(\Grad;#3)}
% \newcommand{\Hcgen}[3]{\overset{#2}{\Sobolev}{}_{#1}(\curl;#3)}
% \newcommand{\HCgen}[3]{\overset{#2}{\Sobolev}{}_{#1}(\Curl;#3)}
% \newcommand{\Hdgen}[3]{\overset{#2}{\Sobolev}{}_{#1}(\div;#3)}
% \newcommand{\HDgen}[3]{\overset{#2}{\Sobolev}{}_{#1}(\Div;#3)}
\newcommand{\Hggen}[3]{\overset{#2}{\Sobolev}(\grad;#3)}
\newcommand{\HGgen}[3]{\overset{#2}{\Sobolev}(\Grad;#3)}
\newcommand{\Hcgen}[3]{\overset{#2}{\Sobolev}(\curl_{#1};#3)}
\newcommand{\HCgen}[3]{\overset{#2}{\Sobolev}(\Curl_{#1};#3)}
\newcommand{\Hdgen}[3]{\overset{#2}{\Sobolev}(\div_{#1};#3)}
\newcommand{\HDgen}[3]{\overset{#2}{\Sobolev}(\Div_{#1};#3)}
\newcommand{\HCsymgen}[3]{\overset{#2}{\Sobolev}{}_{\sym}(\Curl_{#1};#3)}
\newcommand{\Hgom}{\Hggen{}{}{\om}}
\newcommand{\HGom}{\HGgen{}{}{\om}}
\newcommand{\Hcom}{\Hcgen{}{}{\om}}
\newcommand{\HCom}{\HCgen{}{}{\om}}
\newcommand{\Hdom}{\Hdgen{}{}{\om}}
\newcommand{\HDom}{\HDgen{}{}{\om}}
\newcommand{\Hgcom}{\Hggen{}{\circ}{\om}}
\newcommand{\HGcom}{\HGgen{}{\circ}{\om}}
\newcommand{\Hccom}{\Hcgen{}{\circ}{\om}}
\newcommand{\HCcom}{\HCgen{}{\circ}{\om}}
\newcommand{\Hdcom}{\Hdgen{}{\circ}{\om}}
\newcommand{\HDcom}{\HDgen{}{\circ}{\om}}
\newcommand{\Hczom}{\Hcgen{0}{}{\om}}
\newcommand{\HCzom}{\HCgen{0}{}{\om}}
\newcommand{\Hdzom}{\Hdgen{0}{}{\om}}
\newcommand{\HDzom}{\HDgen{0}{}{\om}}
\newcommand{\Hcczom}{\Hcgen{0}{\circ}{\om}}
\newcommand{\HCczom}{\HCgen{0}{\circ}{\om}}
\newcommand{\Hdczom}{\Hdgen{0}{\circ}{\om}}
\newcommand{\HDczom}{\HDgen{0}{\circ}{\om}}
\newcommand{\Hgcgatom}{\Hggen{}{\circ}{\gat,\om}}
\newcommand{\Hgcganom}{\Hggen{}{\circ}{\gan,\om}}
\newcommand{\HGcgatom}{\HGgen{}{\circ}{\gat,\om}}
\newcommand{\HGcganom}{\HGgen{}{\circ}{\gan,\om}}
\newcommand{\Hccgatom}{\Hcgen{}{\circ}{\gat,\om}}
\newcommand{\HCcgatom}{\HCgen{}{\circ}{\gat,\om}}
\newcommand{\Hdcgatom}{\Hdgen{}{\circ}{\gat,\om}}
\newcommand{\Hdcganom}{\Hdgen{}{\circ}{\gan,\om}}
\newcommand{\HDcganom}{\HDgen{}{\circ}{\gan,\om}}
\newcommand{\Hcczgatom}{\Hcgen{0}{\circ}{\gat,\om}}
\newcommand{\HCczgatom}{\HCgen{0}{\circ}{\gat,\om}}
\newcommand{\Hdczganom}{\Hdgen{0}{\circ}{\gan,\om}}
\newcommand{\HDczganom}{\HDgen{0}{\circ}{\gan,\om}}
\newcommand{\Hccganom}{\Hcgen{}{\circ}{\gan,\om}}
\newcommand{\HCcganom}{\HCgen{}{\circ}{\gan,\om}}
\newcommand{\HCsymom}{\HCsymgen{}{}{\om}}
\newcommand{\HCcsymom}{\HCsymgen{}{\circ}{\om}}
\newcommand{\HCcsymgatom}{\HCsymgen{}{\circ}{\gat,\om}}

\newcommand{\Httgen}[2]{\Sobolev{}_{#1}^{-1/2}(\curlga;#2)}
\newcommand{\Httga}{\Httgen{}{\ga}}
\newcommand{\Httgat}{\Httgen{\gat}{\ga}}
\newcommand{\Httgatz}{\Httgen{\gat,0}{\ga}}

\newcommand{\Htgen}[3]{\Sobolev{}_{#1}^{#2}(#3)}
\newcommand{\Htootgen}[2]{\Sobolev{}_{#1}^{1/2}(#2)}
\newcommand{\Htmootgen}[2]{\Sobolev{}_{#1}^{-1/2}(#2)}
\newcommand{\Htootga}{\Htootgen{}{\ga}}
\newcommand{\Htootgan}{\Htootgen{\gan,0}{\ga}}
\newcommand{\Htmootga}{\Htmootgen{}{\ga}}
\newcommand{\Htmootgat}{\Htmootgen{\gat}{\ga}}

\DeclareMathOperator{\XSobolev}{\mathsf{X}}
\DeclareMathOperator{\YSobolev}{\mathsf{Y}}
\newcommand{\xom}{\XSobolev(\om)}
\newcommand{\xqmoom}{\XSobolev^{q-1}(\om)}
\newcommand{\yom}{\YSobolev(\om)}
\newcommand{\yqpoom}{\YSobolev^{q+1}(\om)}
\newcommand{\Xom}{\XSobolev(\om)}
\newcommand{\Yom}{\YSobolev(\om)}
\newcommand{\Xgatnom}{\XSobolev(\gat,\gan,\om)}
\newcommand{\sfS}{\mathsf{S}}
\newcommand{\Som}{\sfS(\om)}
\newcommand{\Szom}{\sfS_{0}(\om)}
\newcommand{\RM}{\mathsf{RM}}
\newcommand{\BD}{\mathsf{BD}}
\newcommand{\BDom}{\BD(\om)}
\newcommand{\BV}{\mathsf{BV}}
\newcommand{\BVom}{\BV(\om)}

\newcommand{\normdst}{\hspace{-0.4ex}}
\newcommand{\scp}[2]{\left\langle#1,#2\right\rangle}
\newcommand{\scps}[2]{\langle#1,#2\rangle}
\newcommand{\scpom}[2]{\scp{#1}{#2}_{\om}}
\newcommand{\scpsom}[2]{\scps{#1}{#2}_{\om}}
\newcommand{\scpLtom}[2]{\scp{#1}{#2}_{\Ltom}}
\newcommand{\scpLtepsom}[2]{\scp{#1}{#2}_{\Ltom,\eps}}
\newcommand{\scpLtepsmoom}[2]{\scp{#1}{#2}_{\Ltom,\eps^{-1}}}
\newcommand{\scpsLtom}[2]{\scps{#1}{#2}_{\Ltom}}
\newcommand{\scpsLtepsom}[2]{\scps{#1}{#2}_{\Ltom,\eps}}
\newcommand{\scpLtqom}[2]{\scp{#1}{#2}_{\Ltqom}}
\newcommand{\scpsLtqom}[2]{\scps{#1}{#2}_{\Ltqom}}
\newcommand{\scpLtqpoom}[2]{\scp{#1}{#2}_{\Ltqpoom}}
\newcommand{\scpsLtqpoom}[2]{\scps{#1}{#2}_{\Ltqpoom}}
\newcommand{\scpLtqmoom}[2]{\scp{#1}{#2}_{\Ltqmoom}}
\newcommand{\scpsLtqmoom}[2]{\scps{#1}{#2}_{\Ltqmoom}}
\newcommand{\scpLtga}[2]{\scp{#1}{#2}_{\Ltga}}
\newcommand{\scpLtgat}[2]{\scp{#1}{#2}_{\Ltgat}}
\newcommand{\norm}[1]{\left|\normdst\left|#1\right|\normdst\right|}
\newcommand{\norms}[1]{|\normdst|#1|\normdst|}
\newcommand{\dnorm}[1]{\left|\normdst\left|\normdst\left|#1\right|\normdst\right|\normdst\right|}
\newcommand{\dnorms}[1]{|\normdst|\normdst|#1|\normdst|\normdst|}
\newcommand{\dnormF}[1]{\dnorm{#1}_{\TF}}
\newcommand{\normom}[1]{\norm{#1}_{\om}}
\newcommand{\normLtom}[1]{\norm{#1}_{\Ltom}}
\newcommand{\normLtepsom}[1]{\norm{#1}_{\Ltom,\eps}}
\newcommand{\normLtepsmoom}[1]{\norm{#1}_{\Ltom,\eps^{-1}}}
\newcommand{\normLtmuom}[1]{\norm{#1}_{\Ltom,\mu}}
\newcommand{\normsLtom}[1]{\norms{#1}_{\Ltom}}
\newcommand{\normsLtepsom}[1]{\norms{#1}_{\Ltom,\eps}}
\newcommand{\normLtqom}[1]{\norm{#1}_{\Ltqom}}
\newcommand{\normsLtqom}[1]{\norms{#1}_{\Ltqom}}
\newcommand{\normLtqpoom}[1]{\norm{#1}_{\Ltqpoom}}
\newcommand{\normsLtqpoom}[1]{\norms{#1}_{\Ltqpoom}}
\newcommand{\normLtqmoom}[1]{\norm{#1}_{\Ltqmoom}}
\newcommand{\normsLtqmoom}[1]{\norms{#1}_{\Ltqmoom}}

\newtheorem{lem}{Lemma}%[section]
\newtheorem{defi}[lem]{Definition}
\newtheorem{theo}[lem]{Theorem}
\newtheorem{cor}[lem]{Corollary}
\newtheorem{rem}[lem]{Remark}
\newtheorem{pro}[lem]{Proposition}
\newtheorem{ass}{Assumption}
\newtheorem{asscount}[lem]{Assumption}
\newtheorem{ex}{Example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclareMathOperator{\rotspace}{\mathsf{R}}
\newcommand{\rotgen}[2]{\overset{#2}{\rotspace}{}_{#1}}
\newcommand{\rotgenom}[2]{\rotgen{#1}{#2}(\om)}
\newcommand{\rom}{\rotgenom{}{}}
\newcommand{\rcom}{\rotgenom{}{\circ}}
\newcommand{\rzom}{\rotgenom{0}{}}
\newcommand{\rczom}{\rotgenom{0}{\circ}}

\newcommand{\rcalom}{\cR(\om)}
\newcommand{\rcalcom}{\overset{\circ}{\cR}(\om)}

\DeclareMathOperator{\divspace}{\mathsf{D}}
\newcommand{\divgen}[2]{\overset{#2}{\divspace}{}_{#1}}
\newcommand{\divgenom}[2]{\divgen{#1}{#2}(\om)}
\newcommand{\dom}{\divgenom{}{}}
\newcommand{\dcom}{\divgenom{}{\circ}}
\newcommand{\dzom}{\divgenom{0}{}}
\newcommand{\dczom}{\divgenom{0}{\circ}}
\def\Dom{\dom}
\def\Dzom{\dzom}
\def\omR{\om_{R}}
\def\DomR{\divgen{}{}(\omR)}

\newcommand{\ho}{\Ho}
\newcommand{\hoc}{\Hoc}
\newcommand{\hoom}{\Hoom}
\newcommand{\hocom}{\Hocom}
\newcommand{\htom}{\Htom}
\newcommand{\Htigen}[3]{\overset{#3}{\tilde{\Sobolev}}{}^{#1}_{#2}}
\def\Htoc{\Htigen{1}{}{\circ}}
\def\HtocomR{\Htoc(\omR)}
\def\HoomR{\Ho(\omR)}
\def\HocomR{\Hoc(\omR)}

\DeclareMathOperator{\U}{\mathsf{U}}
\DeclareMathOperator{\V}{\mathsf{V}}
\def\UomR{\U(\omR)}
\def\VomR{\V(\omR)}

\newcommand{\Hil}[1]{\overset{#1}{\Sobolev}}
\newcommand{\Hilom}[1]{\overset{#1}{\Sobolev}(\om)}
\newcommand{\hi}{\Hil{}}
\newcommand{\hio}{\hi_{1}}
\newcommand{\hit}{\hi_{2}}
\newcommand{\hic}{\Hil{\circ}}
\newcommand{\hiom}{\Hilom{}}
\newcommand{\hicom}{\Hilom{\circ}}

\DeclareMathOperator{\harmonic}{\mathcal{H}}
\newcommand{\harm}[2]{\harmonic^{#1}_{#2}}
\newcommand{\harmom}[2]{\harm{#1}{#2}(\om)}
\newcommand{\harmdom}{\harmom{}{\mathtt{D}}}
\newcommand{\harmdepsom}{\harmom{}{\mathtt{D},\eps}}
\newcommand{\harmdmuom}{\harmom{}{\mathtt{D},\mu}}
\newcommand{\harmdidom}{\harmom{}{\mathtt{D},\id}}
\newcommand{\harmnom}{\harmom{}{\mathtt{N}}}
\newcommand{\harmnepsom}{\harmom{}{\mathtt{N},\eps}}
\newcommand{\harmnmuom}{\harmom{}{\mathtt{N},\mu}}
\newcommand{\harmnidom}{\harmom{}{\mathtt{N},\id}}

\newcommand{\non}{\nonumber}

\newcommand{\pid}{\pi_{\mathtt{D}}}
\newcommand{\pin}{\pi_{\mathtt{N}}}

\newcommand{\scpsiLtom}[2]{\scp{#1}{#2}_{\om}} % simple
\newcommand{\scpsiLtepsom}[2]{\scp{#1}{#2}_{\om,\eps}}
\newcommand{\scpsiLtepsmoom}[2]{\scp{#1}{#2}_{\om,\epsmo}}
\newcommand{\scpsiLtga}[2]{\scps{#1}{#2}_{\ga}}

\newcommand{\scpsoms}[2]{\scps{#1}{#2}_{\oms}}
\newcommand{\scpsepsom}[2]{\scps{#1}{#2}_{\om,\eps}}
\newcommand{\scpsepsoms}[2]{\scps{#1}{#2}_{\oms,\eps}}
\newcommand{\scpsepsmoom}[2]{\scps{#1}{#2}_{\om,\epsmo}}
\newcommand{\scpsepsmooms}[2]{\scps{#1}{#2}_{\oms,\epsmo}}
\newcommand{\scpsmuom}[2]{\scps{#1}{#2}_{\om,\mu}}
\newcommand{\scpsmuoms}[2]{\scps{#1}{#2}_{\oms,\mu}}
\newcommand{\scpsmumoom}[2]{\scps{#1}{#2}_{\om,\mumo}}
\newcommand{\scpsmumooms}[2]{\scps{#1}{#2}_{\oms,\mumo}}

\newcommand{\normo}[1]{\left|#1\right|} % one bar
\newcommand{\normos}[1]{|#1|} % one bar small

\newcommand{\normoLtom}[1]{\normo{#1}_{\Ltom}} % one bar L^2
\newcommand{\normoom}[1]{\normo{#1}_{\om}} % one bar simple
\newcommand{\normosom}[1]{\normos{#1}_{\om}} % one bar small simple

\newcommand{\normoLtepsom}[1]{\normo{#1}_{\om,\eps}}
\newcommand{\normoLtepsoms}[1]{\normo{#1}_{\oms,\eps}}
\newcommand{\normoLtmuom}[1]{\normo{#1}_{\om,\mu}}
\newcommand{\normoLtmuoms}[1]{\normo{#1}_{\oms,\mu}}
\newcommand{\normoLtepsmoom}[1]{\normo{#1}_{\om,\epsmo}}
\newcommand{\normoLtepsmooms}[1]{\normo{#1}_{\oms,\epsmo}}
\newcommand{\normoLtmumoom}[1]{\normo{#1}_{\om,\mumo}}
\newcommand{\normoLtmumooms}[1]{\normo{#1}_{\oms,\mumo}}
\newcommand{\normoepsom}[1]{\normo{#1}_{\om,\eps}}
\newcommand{\normosepsom}[1]{\normos{#1}_{\om,\eps}}
\newcommand{\normoepsoms}[1]{\normo{#1}_{\oms,\eps}}
\newcommand{\normosepsoms}[1]{\normos{#1}_{\oms,\eps}}
\newcommand{\normomuom}[1]{\normo{#1}_{\om,\mu}}
\newcommand{\normosmuom}[1]{\normos{#1}_{\om,\mu}}
\newcommand{\normomuoms}[1]{\normo{#1}_{\oms,\mu}}
\newcommand{\normosmuoms}[1]{\normos{#1}_{\oms,\mu}}
\newcommand{\normoepsmoom}[1]{\normo{#1}_{\om,\epsmo}}
\newcommand{\normosepsmoom}[1]{\normos{#1}_{\om,\epsmo}}
\newcommand{\normoepsmooms}[1]{\normo{#1}_{\oms,\epsmo}}
\newcommand{\normosepsmooms}[1]{\normos{#1}_{\oms,\epsmo}}
\newcommand{\normomumoom}[1]{\normo{#1}_{\om,\mumo}}
\newcommand{\normosmumoom}[1]{\normos{#1}_{\om,\mumo}}
\newcommand{\normomumooms}[1]{\normo{#1}_{\oms,\mumo}}
\newcommand{\normosmumooms}[1]{\normos{#1}_{\oms,\mumo}}

\newcommand{\normslides}[1]{|#1|}
\newcommand{\scpslides}[2]{\langle#1,#2\rangle}
\newcommand{\normLtomslides}[1]{\normslides{#1}_{\Ltom}}
\newcommand{\scpLtomslides}[2]{\scpslides{#1}{#2}_{\Ltom}}

\newcommand{\tcomp}[1]{#1_{\mathtt{t}}}
\newcommand{\ncomp}[1]{#1_{\mathtt{n}}}
\newcommand{\ttr}[2]{\tcomp{#1}|_{#2}}
\newcommand{\ntr}[2]{\ncomp{#1}|_{#2}}
\newcommand{\ttrG}[1]{\ttr{#1}{\Gamma}}
\newcommand{\ntrG}[1]{\ntr{#1}{\Gamma}}
\newcommand{\trbd}[2]{{#1}|_{#2}}
\newcommand{\trG}[1]{\trbd{#1}{\Gamma}}

\DeclareMathOperator{\diam}{diam}
\newcommand{\diamom}{\diam(\om)}

